Optimizing Index Deployment Order for Evolving OLAP (Extended Version)

Query workloads and database schemas in OLAP applications are becoming increasingly complex. Moreover, the queries and the schemas have to continually \textit{evolve} to address business requirements. During such repetitive transitions, the \textit{order} of index deployment has to be considered while designing the physical schemas such as indexes and MVs. An effective index deployment ordering can produce (1) a prompt query runtime improvement and (2) a reduced total deployment time. Both of these are essential qualities of design tools for quickly evolving databases, but optimizing the problem is challenging because of complex index interactions and a factorial number of possible solutions. We formulate the problem in a mathematical model and study several techniques for solving the index ordering problem. We demonstrate that Constraint Programming (CP) is a more flexible and efficient platform to solve the problem than other methods such as mixed integer programming and A* search. In addition to exact search techniques, we also studied local search algorithms to find near optimal solution very quickly. Our empirical analysis on the TPC-H dataset shows that our pruning techniques can reduce the size of the search space by tens of orders of magnitude. Using the TPC-DS dataset, we verify that our local search algorithm is a highly scalable and stable method for quickly finding a near-optimal solution.

==> mip.tex <==
% \section{Problems of Using MIP}
% \label{s:mip}
% % \sectionheadline{MIP (and A*) is completely ill-suited to the problem because
% % the model is not linear.}
% 
% In physical database designs and
% many other fields in computer science, it is a quite common and natural
% choice to solve an optimization problem with Branch-Bound based algorithm
% like MIP or A* search~\cite{papadomanolakis2007ilp, gupta1999selection,
% kimura2010coradd}.
% 
% However, when we tried to solve our problem with MIP, we found
% fundamental mismatches in both modeling and optimization
% mainly caused by the non-linear nature of the problem.
% In this section, we discuss why the problem is ill-suited to
% an MIP approach and explore the desiderata for an alternative approach to solve
% the problem.
% 
% % \headline{Intro:} we tried to solve the problem as an MIP. observed
% % fundamental problems.
% 
% % \headline{Summarize:} Modeling problems and performance problems. 
% 
% \subsection{Modeling Problems}
% \label{s:mip:model}
% To solve the problem in an MIP solver, we need to translate
% the mathematical model defined in Section~\ref{s:definition:model}
% to an integer linear system.
% 
% However, the problem contains completely non-linear constraints and objective
% which cannot be expressed in MIP.
% 
% One example is the constraint for index creation costs. (\ref{e:ccon}) in
% Secttion~\ref{s:definition:model} defines a constraint ``$C_{T_i}=\ldots$''.
% As $T_i$ is also a variable, this constraint is non-linear and cannot be
% expressed as a linear equation.
% 
% Another example is the objective $R_{i-1} C_i$. Here, both $R$ and $C$ are
% variables. Optimizing on a product of variables (which is of course non-linear)
% is impossible in MIP.
% 
% %\headline{Non-linear constraints:}
% % $C_{T_i}=\ldots$ is impossible to express in MIP because $T_i$ is also a
% % variable.
% 
% % \headline{Non-linear objective:} $R_{i-1} C_i$ is impossible to express in
% % MIP because both R and C are variables.
% 
% % \headline{Why it's not allowed:} MIP assumes linear model.
% 
% The fundamental problem is that MIP assumes linear objectives and constraints.
% Non-linear constraints and objectives cannot be modeled as a solvable system.
% 
% \subsection{Performance Problems}
% \label{s:mip:performance}
% 
% Although not straightforward, there is some way to solve non-linear problem
% in MIP (TODO: some citation in OR community that tries it).
% In our case, the only known method is to \textit{discretize} the entire
% span to a limited number of uniform timesteps and define the value of each
% variable at each timestep as an independent variable.
% 
% For the full detail of such a discretized model, we refer readers to
% Appendix~\ref{s:appendix:mipfull}. We only summarize the findings in this
% section.
% 
% % \headline{De-tour:} Discretize and have constraints each of them. Refer
% % appendix for full model.
% 
% By discretization, we lose
% the accuracy of the system. Furthermore, the much more severe problem is that
% now we have several orders of magnitude more variables and constraints
% compared to the original mathematical model. Because MIP solver takes
% a significantly longer time to check to the consistency of constraints and
% variables, the runtime of MIP becomes unrealistic even for a very small problem.
% 
% % \headline{Accuracy:} because of discretization.
% 
% % \headline{More variables/constraints:} orders of magnitude more
% % variables and constraints than fundamentally needed by the mathematical model.
% 
% Also, MIP cannot utilize its most fundamental
% optimization to this problem; Branch-Bound. The performance of MIP highly
% depends on how tightly it can prune
% out bad branches whose relaxed objective value is below the current integer
% solution. However, because our problem has several non-linear properties,
% there is no meaningful linear relaxation.
% 
% \textbf{TODO Figure to show meaningless relaxation. empty rectangle.}
% 
% This problem also applies to A* search and other Branch-Bound based algorithm.
% As we can infer almost nothing in the heuristic distance function,
% A* search needs to check almost all branches except the ones very close to the
% leaves.
% 
% Instead of the linear relaxation, there are the additional
% constraints which can effectively shrink the search space described in
% Section~\ref{s:definition:optimization}.
% However, the additional constraints actually make the runtime of MIP worse, not
% better. Although theoretically the constraints can prune out a part of search
% space, they introduce many more constraints and further slow down
% the consistency check and confuse the MIP solver.
% (TODO : experimental result?)
% 
% % \headline{No pruning:} No pruning by B-B. Illustrate how LB is loose in this
% % model. No meaningful relaxation possible. Also mention the same problem to A*.
% 
% These problems result in totally unrealistic runtimes even for small problems as
% verified in the experimental section.
% 
% % \headline{Evidence:} Refer experimental section and appendix for its
% % terrible performance.
% 
% \subsection{Observation}
% \label{s:mip:conclusion}
% In summary, MIP is fundamentally ill-suited to our problem for the following
% reasons.
% 
% Problem 1: MIP cannot effciently interpret non-linear constraints and
% objectives
% 
% Problem 2: Linear relaxation has no pruning power
% 
% Problem 3: MIP cannot utilize the additional constraints
% 
% Conversely, the desiderata for a platform to efficiently solve the problem
% is as follows.
% 
% Desideratum 1: Can efficiently interpret constraints and objectives
% specific to our problem
% 
% Desideratum 2: Can flexibly control the search strategy with the
% additional constraints
% 
% The first desideratum
% 
% % We note that we devised a relaxation method for the problem at the root node
% % in Section~\ref{s:lns:lb}, but this method cannot relax the problem at
% % arbitrary branch either.
%  
% % \headline{Repeat/Summarize:} Why MIP/A* is fundamentally ill-suited. What are
% % the desirable properties of solvers for this problem (constraint-based
% % flexible
% % model, a solver optimized for combinatorial problem,
% % whitebox optimization, etc). Next section shows CP provides them.
% 
% 
% 
% % \headline{Need for flexible control on optimization:} We know the problem
% % better than the solver. MIP is blackbox. we can't specify how it should be
% % solved.

